Stable Quantum-Correlated Many Body States through Engineered Dissipation

Engineered dissipative reservoirs have the potential to steer many-body quantum systems toward correlated steady states useful for quantum simulation of high-temperature superconductivity or quantum magnetism. Using up to 49 superconducting qubits, we prepared low-energy states of the transverse-field Ising model through coupling to dissipative auxiliary qubits. In one dimension, we observed long-range quantum correlations and a ground-state fidelity of 0.86 for 18 qubits at the critical point. In two dimensions, we found mutual information that extends beyond nearest neighbors. Lastly, by coupling the system to auxiliaries emulating reservoirs with different chemical potentials, we explored transport in the quantum Heisenberg model. Our results establish engineered dissipation as a scalable alternative to unitary evolution for preparing entangled many-body states on noisy quantum processors.

==> authors.tex <==
\begin{flushleft}
    {\hypertarget{authorlist}{${}^\dagger$}  \small Google Quantum AI and Collaborators}

    \bigskip

    \renewcommand{\author}[2]{#1\textsuperscript{\textrm{\scriptsize #2}}}
    \renewcommand{\affiliation}[2]{\textsuperscript{\textrm{\scriptsize #1} #2} \\}
    \newcommand{\corrauthora}[2]{#1$^{\textrm{\scriptsize #2}, \hyperlink{corra}{\ddagger}}$}
    \newcommand{\corrauthorb}[2]{#1$^{\textrm{\scriptsize #2}, \hyperlink{corrb}{\mathsection}}$}
    \newcommand{\xGoogle}{\affiliation{1}{Google Research, Mountain View, CA, USA}}


\newcommand{\xGeneva}{\affiliation{2}{Department of Theoretical Physics, University of Geneva, Quai Ernest-Ansermet 30, 1205 Geneva, Switzerland}}

\newcommand{\xUMass}{\affiliation{3}{Department of Electrical and Computer Engineering, University of Massachusetts, Amherst, MA, USA}}

\newcommand{\xAU}{\affiliation{4}{Department of Electrical and Computer Engineering, Auburn University, Auburn, AL, USA}}

\newcommand{\xCQC}{\affiliation{5}{QSI, Faculty of Engineering \& Information Technology, University of Technology Sydney, NSW, Australia}}

\newcommand{\xUCR}{\affiliation{6}{Department of Electrical and Computer Engineering, University of California, Riverside, CA, USA}}

\newcommand{\xCU}{\affiliation{7}{Department of Chemistry, Columbia University, New York, NY, USA}}

\newcommand{\xUoCA}{\affiliation{8}{Department of Physics and Astronomy, University of California, Riverside, CA, USA}}

\begin{footnotesize}

% Make sure the numbers match up ^^ vv
\newcommand{\Google}{1}
\newcommand{\Geneva}{2}
\newcommand{\UMass}{3}
\newcommand{\AU}{4}
\newcommand{\CQC}{5}
\newcommand{\UCR}{6}
\newcommand{\CU}{7}
\newcommand{\UoCA}{8}


\author{X. Mi}{\Google},
\author{A. A. Michailidis}{\Geneva},
\author{S. Shabani}{\Google},
\author{K. C.~Miao}{\Google},
\author{P. V.~Klimov}{\Google},
\author{J. Lloyd}{\Geneva},
\author{E. Rosenberg}{\Google},
\author{R. Acharya}{\Google},
\author{I. Aleiner}{\Google},
\author{T. I. Andersen}{\Google},
\author{M. Ansmann}{\Google},
\author{F. Arute}{\Google},
\author{K. Arya}{\Google},
\author{A. Asfaw}{\Google},
\author{J. Atalaya}{\Google},
\author{J. C.~Bardin}{\Google,\! \UMass},
\author{A. Bengtsson}{\Google},
\author{G. Bortoli}{\Google},
\author{A. Bourassa}{\Google},
\author{J. Bovaird}{\Google},
\author{L. Brill}{\Google},
\author{M. Broughton}{\Google},
\author{B. B.~Buckley}{\Google},
\author{D. A.~Buell}{\Google},
\author{T. Burger}{\Google},
\author{B. Burkett}{\Google},
\author{N. Bushnell}{\Google},
\author{Z. Chen}{\Google},
\author{B. Chiaro}{\Google},
\author{D. Chik}{\Google},
\author{C. Chou}{\Google},
\author{J. Cogan}{\Google},
\author{R. Collins}{\Google},
\author{P. Conner}{\Google},
\author{W. Courtney}{\Google},
\author{A. L. Crook}{\Google},
\author{B. Curtin}{\Google},
\author{A. G.~Dau}{\Google},
\author{D. M.~Debroy}{\Google},
\author{A. Del~Toro~Barba}{\Google},
\author{S. Demura}{\Google},
\author{A. Di Paolo}{\Google},
\author{I. K. Drozdov}{\Google},
\author{A. Dunsworth}{\Google},
\author{C. Erickson}{\Google},
\author{L. Faoro}{\Google},
\author{E. Farhi}{\Google},
\author{R. Fatemi}{\Google},
\author{V. S.~Ferreira}{\Google},
\author{L. F.~Burgos}{\Google}
\author{E. Forati}{\Google},
\author{A. G.~Fowler}{\Google},
\author{B. Foxen}{\Google},
\author{\'{E}. Genois}{\Google},
\author{W. Giang}{\Google},
\author{C. Gidney}{\Google},
\author{D. Gilboa}{\Google},
\author{M. Giustina}{\Google},
\author{R. Gosula}{\Google},
\author{J. A.~Gross}{\Google},
\author{S. Habegger}{\Google},
\author{M. C.~Hamilton}{\Google,\! \AU},
\author{M. Hansen}{\Google},
\author{M. P.~Harrigan}{\Google},
\author{S. D. Harrington}{\Google},
\author{P. Heu}{\Google},
\author{M. R.~Hoffmann}{\Google},
\author{S. Hong}{\Google},
\author{T. Huang}{\Google},
\author{A. Huff}{\Google},
\author{W. J. Huggins}{\Google},
\author{L. B.~Ioffe}{\Google},
\author{S. V.~Isakov}{\Google},
\author{J. Iveland}{\Google},
\author{E. Jeffrey}{\Google},
\author{Z. Jiang}{\Google},
\author{C. Jones}{\Google},
\author{P. Juhas}{\Google},
\author{D. Kafri}{\Google},
\author{K. Kechedzhi}{\Google},
\author{T. Khattar}{\Google},
\author{M. Khezri}{\Google},
\author{M. Kieferov\'a}{\Google,\! \CQC},
\author{S. Kim}{\Google},
\author{A. Kitaev}{\Google},
\author{A. R.~Klots}{\Google},
\author{A. N.~Korotkov}{\Google,\! \UCR},
\author{F. Kostritsa}{\Google},
\author{J.~M.~Kreikebaum}{\Google},
\author{D. Landhuis}{\Google},
\author{P. Laptev}{\Google},
\author{K.-M. Lau}{\Google},
\author{L. Laws}{\Google},
\author{J. Lee}{\Google,\! \CU},
\author{K. W.~Lee}{\Google},
\author{Y. D. Lensky}{\Google},
\author{B. J.~Lester}{\Google},
\author{A. T.~Lill}{\Google},
\author{W. Liu}{\Google},
\author{A. Locharla}{\Google},
\author{F. D. Malone}{\Google},
\author{O. Martin}{\Google},
\author{J. R.~McClean}{\Google},
\author{M. McEwen}{\Google},
\author{A. Mieszala}{\Google},
\author{S. Montazeri}{\Google},
\author{A. Morvan}{\Google},
\author{R. Movassagh}{\Google},
\author{W. Mruczkiewicz}{\Google},
% \author{O. Naaman}{\Google},
\author{M. Neeley}{\Google},
\author{C. Neill}{\Google},
\author{A. Nersisyan}{\Google},
\author{M. Newman}{\Google},
\author{J. H. Ng}{\Google},
\author{A. Nguyen}{\Google},
\author{M. Nguyen}{\Google},
\author{M. Y. Niu}{\Google},
\author{T. E.~O'Brien}{\Google},
\author{A. Opremcak}{\Google},
\author{A. Petukhov}{\Google},
\author{R. Potter}{\Google},
\author{L. P.~Pryadko}{\Google,\!\UoCA},
\author{C. Quintana}{\Google},
\author{C. Rocque}{\Google},
\author{N. C.~Rubin}{\Google},
\author{N. Saei}{\Google},
\author{D. Sank}{\Google},
\author{K. Sankaragomathi}{\Google},
\author{K. J.~Satzinger}{\Google},
\author{H. F.~Schurkus}{\Google},
\author{C. Schuster}{\Google},
\author{M. J.~Shearn}{\Google},
\author{A. Shorter}{\Google},
\author{N. Shutty}{\Google},
\author{V. Shvarts}{\Google},
\author{J. Skruzny}{\Google},
\author{W. C. Smith}{\Google},
\author{R. Somma}{\Google},
\author{G. Sterling}{\Google},
\author{D. Strain}{\Google},
\author{M. Szalay}{\Google},
\author{A. Torres}{\Google},
\author{G. Vidal}{\Google},
\author{B. Villalonga}{\Google},
\author{C. V.~Heidweiller}{\Google},
\author{T. White}{\Google},
\author{B. W.~K.~Woo}{\Google},
\author{C. Xing}{\Google},
\author{Z.~J. Yao}{\Google},
\author{P. Yeh}{\Google},
\author{J. Yoo}{\Google},
\author{G. Young}{\Google},
\author{A. Zalcman}{\Google},
\author{Y. Zhang}{\Google},
\author{N. Zhu}{\Google},
\author{N. Zobrist}{\Google},
\author{H. Neven}{\Google},
\author{R. Babbush}{\Google},
\author{D. Bacon}{\Google},
\author{S. Boixo}{\Google},
\author{J. Hilton}{\Google},
\author{E. Lucero}{\Google},
\author{A. Megrant}{\Google},
\author{J. Kelly}{\Google},
\author{Y. Chen}{\Google},
\author{P. Roushan}{\Google},
\author{V. Smelyanskiy}{\Google},
\author{D. A. Abanin}{\Google,\! \Geneva}

\bigskip

\xGoogle
\xGeneva
\xUMass
\xAU
\xCQC
\xUCR
\xCU
\xUoCA

\renewcommand{\Google}{1}
\renewcommand{\Geneva}{2}
\renewcommand{\UMass}{3}
\renewcommand{\AU}{4}
\renewcommand{\CQC}{5}
\renewcommand{\UCR}{6}
\renewcommand{\CU}{7}
\renewcommand{\UoCA}{8}

\end{footnotesize}
\end{flushleft}
